DRL-FAS: A Novel Framework Based on Deep Reinforcement Learning for Face Anti-Spoofing

Inspired by the philosophy employed by human beings to determine whether a presented face example is genuine or not, i.e., to glance at the example globally first and then carefully observe the local regions to gain more discriminative information, for the face anti-spoofing problem, we propose a novel framework based on the Convolutional Neural Network (CNN) and the Recurrent Neural Network (RNN). In particular, we model the behavior of exploring face-spoofing-related information from image sub-patches by leveraging deep reinforcement learning. We further introduce a recurrent mechanism to learn representations of local information sequentially from the explored sub-patches with an RNN. Finally, for the classification purpose, we fuse the local information with the global one, which can be learned from the original input image through a CNN. Moreover, we conduct extensive experiments, including ablation study and visualization analysis, to evaluate our proposed framework on various public databases. The experiment results show that our method can generally achieve state-of-the-art performance among all scenarios, demonstrating its effectiveness.

==> abstract.tex <==



==> exp-oulu-ext-bk.tex <==
\begin{table*}[htbp]
  \centering
  \caption{The comparison between the ResNet18 baseline and our proposed framework. The APCER (\%), BPCER (\%), and ACER (\%) results are reported on the four protocols (P1, P2, P3, P4) of the OULU-NPU database. For the experiments, we set $p=8$ and $T=8$.}
  %\begin{adjustbox}{width=\columnwidth} 
  \begin{tabular}{|c|l|c|c|c|c|l|c|c|c|}
    \hline
    \multicolumn{1}{|l|}{Protocol } & Method & APCER & BPCER & ACER  & \multicolumn{1}{l|}{Protocol } & Method & APCER & BPCER & ACER \bigstrut\\
    \hline
%    \multirow{12}[24]{*}{P1} & DeSpoofing \cite{FAS-DeSpoofing-ECCV-2018} & 1.2   & 1.7   & 1.5   & \multirow{12}[24]{*}{P2} & DeSpoofing \cite{FAS-DeSpoofing-ECCV-2018} & 4.4   & 4.2   & 4.3 \bigstrut\\
%\cline{2-5}\cline{7-10}          & Auxiliary \cite{FAS-Auxiliary-CVPR-2018} & 1.6 & 1.6 & 1.6 &       & Auxiliary \cite{FAS-Auxiliary-CVPR-2018} & 2.7 & 2.7 & 2.7 \bigstrut\\
\multirow{12}[24]{*}{P1}         & ResNet18 ($\alpha=0.0$) & 6.6 & 1.4 & 4.0 & \multirow{12}[24]{*}{P2}      & ResNet18 ($\alpha=0.0$) & 6.8 & 2.1 & 4.5 \bigstrut\\
\cline{2-5}\cline{7-10}          & ResNet18 ($\alpha=0.2$) & 8.0 & 2.6 & 5.3 &       & ResNet18 ($\alpha=0.2$) & 4.7 & 2.0 & 3.3 \bigstrut\\
\cline{2-5}\cline{7-10}          & ResNet18 ($\alpha=0.4$) & 2.9 & 1.9 & 2.4 &       & ResNet18 ($\alpha=0.4$) & 6.1 & 1.0 & 3.6 \bigstrut\\
\cline{2-5}\cline{7-10}          & ResNet18 ($\alpha=0.6$) & 1.2 & 3.4 & 2.3 &       & ResNet18 ($\alpha=0.6$) & 6.9 & 1.4 & 3.7 \bigstrut\\
\cline{2-5}\cline{7-10}          & ResNet18 (FULL) & 14.4 & 0.0 & 7.2 &       & ResNet18 (FULL) & 2.8 & 1.8 & 2.3 \bigstrut\\
\cline{2-5}\cline{7-10}          & Ours ($\alpha=0.0$) & 6.2 & 1.2 & 3.7 &       & Ours ($\alpha=0.0$) & 6.6  & 1.3  & 4.0 \bigstrut\\
\cline{2-5}\cline{7-10}          & Ours ($\alpha=0.2$) & 7.9 & 0.8 & 4.4 &       & Ours ($\alpha=0.2$) & 5.3  & 0.8 & 3.0 \bigstrut\\
\cline{2-5}\cline{7-10}          & Ours ($\alpha=0.4$) & 1.6 & 1.6 & 1.6 &       & Ours ($\alpha=0.4$) & 3.8   & 3.0     & 3.4 \bigstrut\\
\cline{2-5}\cline{7-10}          & Ours ($\alpha=0.6$) & 2.5 & 0.3 & \textbf{1.4} &       & Ours ($\alpha=0.6$) & 4.4  & 0.8 & 2.6 \bigstrut\\
\cline{2-5}\cline{7-10}          & Ours (FULL) & 5.4 & 4.0 & 4.7 &       & Ours (FULL) & 3.7   & 0.1   & \textbf{1.9} \bigstrut\\
    \hline
   % \multirow{12}[24]{*}{P3} & DeSpoofing \cite{FAS-DeSpoofing-ECCV-2018} & 4.0$\pm$1.8 & 3.8$\pm$1.2 & 3.6$\pm$1.6 & \multirow{12}[24]{*}{P4} & DeSpoofing \cite{FAS-DeSpoofing-ECCV-2018} & 5.1$\pm$6.3 & 6.1$\pm$5.1 & 5.6$\pm$5.7 \bigstrut\\
%\cline{2-5}\cline{7-10}          & Auxiliary \cite{FAS-Auxiliary-CVPR-2018} & 2.7$\pm$1.3 & 3.1$\pm$1.7 & 2.9$\pm$1.5 &       & Auxiliary \cite{FAS-Auxiliary-CVPR-2018} & 9.3$\pm$5.6 & 10.4$\pm$6.0 & 9.5$\pm$6.0 \bigstrut\\
%\cline{2-5}\cline{7-10}          & ResNet18 ($\alpha=0.0$) & 4.9$\pm$6.0 & 9.3$\pm$15.3 & 7.2$\pm$7.0 &       & ResNet18 ($\alpha=0.0$) & 12.1$\pm$11.1 & 8.7$\pm$10.9 & 10.4$\pm$6.0 \bigstrut\\
\multirow{12}[24]{*}{P3}        & ResNet18 ($\alpha=0.0$) & 4.9$\pm$6.0 & 9.3$\pm$15.3 & 7.2$\pm$7.0 &  \multirow{12}[24]{*}{P4}      & ResNet18 ($\alpha=0.0$) & 12.1$\pm$11.1 & 8.7$\pm$10.9 & 10.4$\pm$6.0 \bigstrut\\
\cline{2-5}\cline{7-10}          & ResNet18 ($\alpha=0.2$) & 3.8$\pm$3.1 & 5.8$\pm$11.3 & 4.8$\pm$5.0 &       & ResNet18 ($\alpha=0.2$) & 10.1$\pm$8.4 & 8.7$\pm$16.4 & 9.4$\pm$7.1 \bigstrut\\
\cline{2-5}\cline{7-10}          & ResNet18 ($\alpha=0.4$) & 3.4$\pm$3.2 & 5.6$\pm$9.4 & 4.5$\pm$4.1 &       & ResNet18 ($\alpha=0.4$) & 10.2$\pm$7.6 & 4.5$\pm$7.5 & 7.4$\pm$3.8 \bigstrut\\
\cline{2-5}\cline{7-10}          & ResNet18 ($\alpha=0.6$) & 5.4$\pm$5.2 & 4.7$\pm$5.3 & 5.1$\pm$2.4 &       & ResNet18 ($\alpha=0.6$) & 9.9$\pm$6.6 & 2.7$\pm$2.2 & 6.3$\pm$2.6 \bigstrut\\
\cline{2-5}\cline{7-10}          & ResNet18 (FULL) & 2.2$\pm$2.1 & 4.6$\pm$3.1 & 3.4$\pm$1.3 &       & ResNet18 (FULL) & 21.0$\pm$11.8 & 1.9$\pm$2.6 & 11.4$\pm$5.1 \bigstrut\\
\cline{2-5}\cline{7-10}          & Ours ($\alpha=0.0$) & 3.7$\pm$5.1 & 9.1$\pm$14.7 & 6.4$\pm$6.9 &       & Ours ($\alpha=0.0$) & 10.8$\pm$11.1 & 8.3$\pm$12.1 & 9.5$\pm$6.6 \bigstrut\\
\cline{2-5}\cline{7-10}          & Ours ($\alpha=0.2$) & 2.7$\pm$1.4 & 5.1$\pm$5.2 & 3.9$\pm$2.3 &       & Ours ($\alpha=0.2$) & 10.5$\pm$8.4 & 6.8$\pm$13.2 & 8.6$\pm$5.6 \bigstrut\\
\cline{2-5}\cline{7-10}          & Ours ($\alpha=0.4$) & 4.1$\pm$2.5 & 1.6$\pm$1.8 & \textbf{2.9}$\pm$1.4 &       & Ours ($\alpha=0.4$) & 5.4$\pm$6.0 & 6.7$\pm$10.6 & 6.0$\pm$4.6 \bigstrut\\
\cline{2-5}\cline{7-10}          & Ours ($\alpha=0.6$) & 3.6$\pm$2.6 & 2.6$\pm$3.3 & 3.1$\pm$1.8 &       & Ours ($\alpha=0.6$) & 9.1$\pm$7.3 & 0.8$\pm$1.8 & \textbf{5.0}$\pm$3.7\bigstrut\\
\cline{2-5}\cline{7-10}          & Ours (FULL) & 4.6$\pm$3.6 & 1.3$\pm$1.8 & 3.0$\pm$1.5 &       & Ours (FULL) & 8.1$\pm$2.7 & 6.9$\pm$5.8 & 7.2$\pm$3.9 \bigstrut\\
    \hline
    \end{tabular}%
%\end{adjustbox}
    \label{tab-oulu-ext}%
\end{table*}%




==> exp-oulu2.tex <==
\begin{table*}[htbp]
  \raggedright
  %
  \begin{threeparttable}
  \caption{Experiment results on the OULU-NPU for the 4 protocols. Results are in terms of EER (\%) on the deveopment (Dev) set, and in terms of APCER (\%), BPCER (\%) and ACER (\%) on the testing (Test) set. }
  
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{Protocol}} & \multirow{2}[4]{*}{Method} & Dev   & \multicolumn{3}{c|}{\centering Test} & \multicolumn{1}{c|}{\multirow{2}[4]{*}{Protocol}} & \multirow{2}[4]{*}{Method } & Dev   & \multicolumn{3}{c|}{Test} \bigstrut\\
\cline{3-6}\cline{9-12}          & \multicolumn{1}{c|}{} & EER   & APCER & BPCER & ACER  &       & \multicolumn{1}{c|}{} & EER   & APCER  & BPCER & ACER \bigstrut\\
    \hline
    \multirow{7}[14]{*}{1} & CpqD \cite{FAS-Competetion-IJCB-2017} & \multicolumn{1}{c|}{0.6} & \multicolumn{1}{c|}{2.9} & \multicolumn{1}{c|}{10.8} & \multicolumn{1}{c|}{6.9} & \multirow{7}[14]{*}{2} & MixedFASNet\cite{FAS-Competetion-IJCB-2017}  & \multicolumn{1}{c|}{1.3} & \multicolumn{1}{c|}{9.7} & \multicolumn{1}{c|}{2.5} & \multicolumn{1}{c|}{6.1} \bigstrut\\
\cline{2-6}\cline{8-12}          & GRADANT \cite{FAS-Competetion-IJCB-2017}  & \multicolumn{1}{c|}{1.1} & \multicolumn{1}{c|}{1.3} & \multicolumn{1}{c|}{12.5} & \multicolumn{1}{c|}{6.9} &       & GRADANT\cite{FAS-Competetion-IJCB-2017}  & \multicolumn{1}{c|}{0.9} & \multicolumn{1}{c|}{3.1} & \multicolumn{1}{c|}{1.9} & \multicolumn{1}{c|}{2.5} \bigstrut\\
\cline{2-6}\cline{8-12}          & DeSpoofing\cite{FAS-DeSpoofing-ECCV-2018}  & $-$     & \multicolumn{1}{c|}{\textbf{1.2}} & \multicolumn{1}{c|}{\textbf{1.7}} & \multicolumn{1}{c|}{\textbf{1.5}} &       & DeSpoofing\cite{FAS-DeSpoofing-ECCV-2018}  & $-$    & \multicolumn{1}{c|}{4.2} & \multicolumn{1}{c|}{4.4} & \multicolumn{1}{c|}{4.3} \bigstrut\\
\cline{2-6}\cline{8-12}  & Auxiliary\cite{FAS-Auxiliary-CVPR-2018} & $-$  & \multicolumn{1}{c|}{1.6} & \multicolumn{1}{c|}{1.6} & \multicolumn{1}{c|}{1.6} &       & Auxiliary\cite{FAS-Auxiliary-CVPR-2018} & $-$ & \multicolumn{1}{c|}{\textbf{2.7}} & \multicolumn{1}{c|}{2.7} & \multicolumn{1}{c|}{2.7} \bigstrut\\
\cline{2-6}\cline{8-12}          & MSR-MobileNet\cite{FAS-MSR-TIFS-2019} & \multicolumn{1}{c|}{5.2} & \multicolumn{1}{c|}{3.9} & \multicolumn{1}{c|}{9.5} & \multicolumn{1}{c|}{6.7} &       & MSR-MobileNet\cite{FAS-MSR-TIFS-2019} & \multicolumn{1}{c|}{5.2} & \multicolumn{1}{c|}{3.9} & \multicolumn{1}{c|}{9.5} & \multicolumn{1}{c|}{6.7} \bigstrut\\
\cline{2-6}\cline{8-12}          & MSR-ResNet\cite{FAS-MSR-TIFS-2019} & \multicolumn{1}{c|}{2.1} & \multicolumn{1}{c|}{5.1} & \multicolumn{1}{c|}{6.7} & \multicolumn{1}{c|}{5.9} &       & MSR-ResNet \cite{FAS-MSR-TIFS-2019} & \multicolumn{1}{c|}{5.2} & \multicolumn{1}{c|}{3.9} & \multicolumn{1}{c|}{9.5} & \multicolumn{1}{c|}{6.7} \bigstrut\\
\cline{2-6}\cline{8-12}          & DRL (ours)  & \multicolumn{1}{c|}{1.8} & \multicolumn{1}{c|}{5.4} & \multicolumn{1}{c|}{4.0} & \multicolumn{1}{c|}{4.7} &       & DRL (ours)  & \multicolumn{1}{c|}{0.5} & \multicolumn{1}{c|}{3.7} & \multicolumn{1}{c|}{\textbf{0.1}} & \multicolumn{1}{c|}{\textbf{1.9}} \bigstrut\\
    \hline
    \multirow{7}[14]{*}{3} & MixedFASNet\cite{FAS-Competetion-IJCB-2017}  & 1.4$\pm$0.5  & 5.3$\pm$6.7  & 7.8$\pm$5.5  & 6.5$\pm$4.6 & \multirow{7}[14]{*}{4} & Massy HNU\cite{FAS-Competetion-IJCB-2017}  & 1.0$\pm$0.4  & 35.8$\pm$35.3  & 8.3$\pm$4.1  & 22.1$\pm$17.6 \bigstrut\\
\cline{2-6}\cline{8-12}          & GRADANT\cite{FAS-Competetion-IJCB-2017}  & 0.9$\pm$0.4  & 2.6$\pm$3.9  & 5.0$\pm$5.3  & 3.8$\pm$2.4 &       & GRADANT\cite{FAS-Competetion-IJCB-2017}  & 1.1$\pm$0.3  & 5.0$\pm$4.5  & 15.0$\pm$7.1  & 10.0$\pm$5.0 \bigstrut\\
\cline{2-6}\cline{8-12}          & DeSpoofing\cite{FAS-DeSpoofing-ECCV-2018}  & $-$     & 4.0$\pm$1.8  & 3.8$\pm$1.2  & 3.6$\pm$1.6 &       & DeSpoofing\cite{FAS-DeSpoofing-ECCV-2018}  & $-$    & 5.1$\pm$6.3  & 6.1$\pm$5.1  & \textbf{5.6}$\pm$5.7 \bigstrut\\
\cline{2-6}\cline{8-12}   & Auxiliary\cite{FAS-Auxiliary-CVPR-2018} & $-$   & \textbf{2.7}$\pm$\textbf{1.3}  & 3.1$\pm$1.7  & \textbf{2.9}$\pm$\textbf{1.5} &       & Auxiliary\cite{FAS-Auxiliary-CVPR-2018} & $-$     & 9.3$\pm$5.6  & 10.4$\pm$6.0  & 9.5$\pm$6.0 \bigstrut\\
\cline{2-6}\cline{8-12}          & MSR-MobileNet\cite{FAS-MSR-TIFS-2019} & 5.1$\pm$0.3  & 8.4$\pm$4.5  & 5.3$\pm$2.3  & 6.3$\pm$2.2 &       & MSR-MobileNet\cite{FAS-MSR-TIFS-2019} & 6.1$\pm$0.7  & 10.9$\pm$4.6  & 12.7$\pm$5.1  & 11.3$\pm$3.9 \bigstrut\\
\cline{2-6}\cline{8-12}          & MSR-ResNet\cite{FAS-MSR-TIFS-2019} & 1.9$\pm$0.4  & 3.9$\pm$2.8  & 7.3$\pm$\textbf{1.1}  & 5.6$\pm$1.6 &       & MSR-ResNet \cite{FAS-MSR-TIFS-2019} & 2.3$\pm$0.3  & 11.9$\pm$3.9  & 9.7$\pm$4.8  & 9.8$\pm$4.2 \bigstrut\\
\cline{2-6}\cline{8-12}          & DRL (ours)  & 0.6$\pm$0.3%0.34  
& 4.6$\pm$3.6  & \textbf{1.3}$\pm$1.8  & 3.0$\pm$\textbf{1.5} &   & DRL (ours)  & 1.8$\pm$0.5%0.21   
& 8.1$\pm$\textbf{2.7} &  6.9$\pm$5.8 &  7.2$\pm$\textbf{3.9} \bigstrut\\
    \hline
    \end{tabular}    
    \begin{tablenotes}
      \item $\bullet$ Protocol 1, 2, 3 is for evaluating a model's generalization capability to unseen sessions, unseen attack mediums, and unseen camera modules respectively. Protocol 4 extends the evaluation to unseen sessions, attack mediums and camera modules at the same time.
      \item $\bullet$ For experiments of Protocol 1 and 2, the testing is only done once so there are no terms of standard deviation.
    \end{tablenotes}
    \end{threeparttable}
  
  \label{tab-exp-oulu}%
\end{table*}%






==> exp-random.tex <==
% \begin{table}[htbp]
%     \centering
%     \caption{The comparison of diffrent methods for selecting patches.}
%       \begin{tabular}{|l|c|c|c|c|}
%       \hline
%       \multicolumn{1}{|c|}{\multirow{2}[4]{*}{Method}} & \multicolumn{1}{c|}{CASIA} & \multicolumn{2}{c|}{CASIA$\rightarrow$REPLAY}       & ROSE-YOUTU \bigstrut\\
%   \cline{2-5}          & \multicolumn{1}{c|}{EER} & \multicolumn{1}{c|}{HTER} & \multicolumn{1}{c|}{AUC} & EER \bigstrut\\
%       \hline
%       Random & 0.32\% & 30.50\% & 0.76 & 2.14\% \bigstrut\\
%       \hline
%       DRL (ours) & 0.17\% & 28.40\% & 0.79  & 1.79\% \bigstrut\\
%       \hline
%       \end{tabular}%
%     \label{tab-r2-selection}%
%   \end{table}%
  % Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[tbp]
%     \centering
%     \caption{The comparison of diffrent methods for selecting patches. The performance is evaluated in terms of EER (\%)}
%       \begin{tabular}{|l|c|c|}
%       \hline
%       Method & RANDOM & DRL (ours) \bigstrut\\
%       \hline
%       CASIA & 0.32 & 0.17 \bigstrut\\
%       \hline
%       REPLAY-ATTAK & 0.00 & 0.00 \bigstrut\\
%       \hline
%       ROSE-YOUTU & 1.79  & 2.14 \bigstrut\\
%       \hline
%       \end{tabular}%
%     \label{tab-r2-selection}%
%   \end{table}%

  % Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{The comparison of different methods for selecting patches. The performance is evaluated in terms of EER (\%). The \textbf{best results} are highlighted in bold. In the experiments, we set $p=8$ and $T=8$.}
     \begin{tabular}{|l|c|c|c|}
    \hline
    EER & MAX-SCORES & RANDOM & DRL (ours) \bigstrut\\
    \hline
    CASIA & 0.25 &0.32 & \textbf{0.17} \bigstrut\\
    \hline
    IDIAP & 0.00 & 0.00 & \textbf{0.00} \bigstrut\\
    \hline
    ROSE-YOUTU & 3.29 & 2.14  & \textbf{1.79} \bigstrut\\
    \hline
    OULU-NPU-P1 & 3.82 &3.57  & \textbf{2.58} \bigstrut\\
    \hline
    OULU-NPU-P2 & 1.54 &1.76  & \textbf{1.15}\bigstrut\\
    \hline
    OULU-NPU-P3 & 1.20$\pm$1.03 & 1.38$\pm$0.94 & \textbf{1.18}$\pm$1.12 \bigstrut\\
    \hline
    OULU-NPU-P4 & 4.67 $\pm$1.31  &4.32$\pm$1.75 & \textbf{3.12}$\pm$2.01 \bigstrut\\
    \hline
    \end{tabular}%
    \label{tab-r2-selection}%
\end{table}%


==> exp-siw.tex <==

	


==> p.tex <==

  

==> parameters.tex <==



==> r3-oulu-extract.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{The comparison of experiment results of the DeSpoofing, Auxiliary, and ours with the }
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\cline{1-1}\cline{3-6}\cline{8-10}    \multicolumn{1}{c|}{\multirow{4}[8]{*}{P1}} & Method & APCER  & BPCER & ACER  & \multirow{4}[8]{*}{P2} & \multicolumn{1}{l|}{Method} & APCER  & BPCER & ACER \bigstrut\\
\cline{2-5}\cline{7-10}    \multicolumn{1}{c|}{} & DeSpoofing & 1.2   & 1.7   & 1.5   &       & DeSpoofing & 4.2   & 4.4   & 4.3 \bigstrut\\
\cline{2-5}\cline{7-10}    \multicolumn{1}{c|}{} & Auxiliary & 1.6   & 1.6   & 1.6   &       & Auxiliary & 2.7   & 2.7   & 2.7 \bigstrut\\
\cline{2-5}\cline{7-10}    \multicolumn{1}{c|}{} & Ours  & 5.4   & 4     & 4.7   &       & Ours  & 3.7   & 0.1   & 0.9 \bigstrut\\
    \hline
    \multirow{4}[8]{*}{P3} & Method & APCER  & BPCER & ACER  & \multirow{4}[8]{*}{P4} & \multicolumn{1}{l|}{Method} & APCER  & BPCER & ACER \bigstrut\\
\cline{2-5}\cline{7-10}          & DeSpoofing & 4     & 3.8   & 3.6   &       & DeSpoofing & 5.1   & 6.1   & 5.6 \bigstrut\\
\cline{2-5}\cline{7-10}          & Auxiliary & 2.7   & 3.1   & 2.9   &       & Auxiliary & 9.3   & 10.4  & 9.5 \bigstrut\\
\cline{2-5}\cline{7-10}          & Ours  & 4.6   & 1.3   & 3     &       & Ours  & 8.1   & 6.8   & 7.2 \bigstrut\\
    \hline
    \end{tabular}%
  \label{r3-oulu-extract}%
\end{table}%

